Chemical Abundances in the Metal-Poor Globular Cluster ESO 280-SC06: A Formerly Massive, Tidally Disrupted Globular Cluster

We present the first high-resolution abundance study of ESO 280-SC06, one of the least luminous and most metal-poor gravitationally bound Milky Way globular clusters. Using Magellan/MIKE spectroscopy for ten stars, we confirm the cluster's low metallicity as [Fe/H] = $-2.54 \pm 0.06$ and the presence of a nitrogen-enhanced star enriched by binary mass transfer. We determine abundances or abundance upper limits for 21 additional elements from the light, alpha, odd-Z, iron peak, and neutron-capture groups for all ten stars. We find no spread in neutron-capture elements, unlike previous trends identified in some metal-poor globular clusters such as M15 and M92. Eight of the ten stars have light-element abundance patterns consistent with second-population globular cluster stars, which is a significantly larger second-population fraction than would be expected from the low present-day mass of $10^{4.1}$ Msun. We estimate the initial mass of the cluster as $10^{5.4 - 5.7}$ Msun based on its orbit in the Milky Way. A preferential loss of first-population stars could explain the high fraction of second-population stars at the present time. Our results emphasize the importance of considering mass loss when studying globular clusters and their enrichment patterns.

==> cluster_abunds.tex <==
element&mean abundance&abundance uplim&abundance lowlim&mean dispersion&dispersion uplim&dispersion lowlim
[Fe/H]&-2.54&0.06&0.06&0.11&nan&nan
[Fe II/H]&-2.55&0.05&0.05&0.1&nan&nan
[C/Fe]&-0.17&0.14&0.13&0.2&0.2&0.15
[N/Fe]&0.95&0.04&0.11&0.29&0.27&0.23
[Na/Fe]&0.84&0.07&0.07&0.18&nan&nan
[Na/Fe], nLTE&0.39&0.07&0.07&0.21&nan&nan
[Mg/Fe]&0.34&0.06&0.06&0.13&nan&nan
[Al/Fe]&0.03&0.17&0.19&0.44&0.22&0.19
[Al/Fe], nLTE, capped&0.84&0.11&0.17&0.41&0.21&0.19
[Si/Fe]&0.59&0.08&0.09&0.14&nan&nan
[K/Fe]&0.7&0.07&0.07&0.12&nan&nan
[Ca/Fe]&0.38&0.06&0.06&0.11&nan&nan
[Sc/Fe II]&0.1&0.06&0.06&0.12&nan&nan
[Ti/Fe]&0.28&0.07&0.07&0.13&nan&nan
[Ti II/Fe II]&0.38&0.07&0.07&0.12&nan&nan
[V/Fe]&0.11&0.1&0.1&0.19&nan&nan
[Cr/Fe]&-0.17&0.07&0.07&0.15&nan&nan
[Mn/Fe]&-0.38&0.08&0.07&0.14&nan&nan
[Co/Fe]&0.16&0.08&0.08&0.14&nan&nan
[Ni/Fe]&0.07&0.07&0.07&0.14&nan&nan
[Zn/Fe]&0.2&0.1&0.09&0.17&nan&nan
[Sr/Fe II]&0.21&0.1&0.1&0.25&nan&nan
[Y/Fe II]&-0.12&0.08&0.08&0.14&nan&nan
[Zr/Fe II]&0.28&0.09&0.09&0.17&nan&nan
[Ba/Fe II]&-0.34&0.06&0.06&0.12&nan&nan
[La/Fe II]&-0.0&0.11&0.12&0.31&nan&nan
[Eu/Fe II]&0.38&0.08&0.08&0.18&nan&nan


==> oldtable.tex <==
%% This is the table sent around in Feb 2021, values are changing a bit so APJ is moving a copy here

\begin{deluxetable*}{lccl}
\tablecolumns{4}
\tablecaption{\label{tab:galprops}Galaxy Properties}
\tablehead{Parameter & Antlia 2 & Crater 2 & Description}
\startdata
% 143.887, -36.767
% -0.0443 +/- 0.0452, +0.0342 +/- 0.0701
% 143.8427 +/- 0.0452, -36.7328 +/- 0.0701
%% NOTE/TODO: THESE NUMBERS HAVE BEEN UPDATED BUT NOT PROPAGATED TO TEXT/FIGURES/ANALYSIS
%   $\alpha$, $\delta$ (deg) & 143.8868, -36.7673 (1) & 177.310, -18.413 (2) & Galaxy center \\
%   $\alpha$, $\delta$ (deg) & $143.8427 \pm 0.0452$, $-36.7673 \pm 0.0701$ & 177.310, -18.413 (2) & Galaxy center \\
  $\alpha$ (deg) & $143.8427 \pm 0.0452$ & 177.310 (2) & Galaxy center RA \\
  $\delta$ (deg) & $-36.7328 \pm 0.0701$ & -18.413 (2) & Galaxy center Dec \\
  $\mu$ (mag) & $20.6 \pm 0.11$ (1) & $20.35 \pm 0.07$ (2,3) & Distance modulus\\
  $d$ (kpc) & 131.8 (1) & 117.5 (2) & Distance \\
  $M_V$ & $-9.37 \pm 0.13$ & $-8.2$ (2) & Luminosity \\
  $r_h$ (arcmin) & $65.2 \pm 4.1$ & $31.2 \pm 2.5$ (2) & Circularized half light radius\\
  $r_h$ (pc) & $2499 \pm 156$ & $1066 \pm 84$ (2) & Circularized half light radius\\
  $a_h$ (arcmin) & TODO & TODO & Half light major axis\\
  $a_h$ (pc) & TODO & TODO (2) & Half light major axis\\
  $e$ ($1-b/a$) & $0.61 \pm 0.03$ & $0.12 \pm 0.02$ (3) & Ellipticity \\
  $\theta_{\text{PA}}$ (deg) & $152.6 \pm 2.1$ & $135 \pm 4$ (3) & Position angle (E. of N.)\\
  $\mu_V$ (mag arcsec$^{-2}$) & $31.2 \pm 0.2$ & $30.6 \pm 0.2$ (2) & Surface brightness within half light radius \\
%   $\alpha$, $\delta$ (deg) & 143.8868, -36.7673 (1) & 177.310, -18.413 (2) & Galaxy center \\
%   $M_V$ & $-9.03$ (1) & $-8.2$ (2) & Luminosity \\
%   $r_h$ (arcmin) & $76.2 \pm 7.2$ (1) & $31.2 \pm 2.5$ (2) & Half light radius\\
%   $e$ ($1-b/a$) & $0.38 \pm 0.08$ (1) & $0.12 \pm 0.02$ (3) & Ellipticity \\
%   $\theta_{\text{PA}}$ (deg) & $156 \pm 6$ (1) & $135 \pm 4$ (3) & Position angle\\
%   $\mu$ (mag) & $20.6 \pm 0.11$ (1) & $20.35 \pm 0.07$ (2,3) & Distance modulus\\
%   $d$ (kpc) & 131.8 (1) & 117.5 (2) & Distance \\
\hline
  $\vhel$ ($\kms$) & $+288.7 ^{+0.4} _{-0.4}$ & $+89.3 ^{+0.3} _{-0.3}$ & Heliocentric radial velocity \\
  %% T19: 290.9; C17/F19: 87.4/87.5
  $\mu_{\alpha^*}$ ($\masyr$) & $-0.094 ^{+0.007} _{-0.007}$ & $-0.073 ^{+0.021} _{-0.021}$ & Heliocentric proper motion, RA $\cos \delta$ \\
  $\mu_{\delta}$ ($\masyr$) & $+0.103 ^{+0.008} _{-0.008}$ & $-0.123 ^{+0.013} _{-0.013}$ & Heliocentric proper motion, Dec.\\
\hline
  $\vgsr$ (\kms) & $49.8^{+0.4}_{-0.4}$ & $-81.4 ^{+0.3} _{-0.3}$ & Galactic standard of rest, radial velocity \\
  $\mu_{\alpha^*,\text{gsr}}$ (\masyr) & $-0.046^{+0.007}_{-0.007}$ & $+0.131 ^{+0.021} _{-0.021}$ & Galactic standard of rest, proper motion, RA $\cos \delta$\\
  $\mu_{\delta,\text{gsr}}$ (\masyr) & $+0.179 ^{+0.008} _{-0.008}$ & $+0.118 ^{+0.013} _{-0.012}$ & Galactic standard of rest, proper motion, Dec\\
  $\sigma_v$ (\kms) & $5.96^{+0.38}_{-0.36}$ & $+2.36 ^{+0.44} _{-0.30}$ & Radial velocity dispersion \\
  %% T19: 5.7 +/- 1.1; C17/F19: 2.8 +/- 0.3, 2.7 +/- 0.5
  $k_v$ (\kms/deg) & $3.75^{+0.63}_{-0.57}$ & $3.76 ^{+1.10} _{-1.08}$ & Linear radial velocity gradient\\
  $k_v$ (\kms/kpc) & $1.63^{+0.27}_{-0.25}$ & $1.83 ^{+0.54}_{-0.52}$ & Linear radial velocity gradient\\
  $\theta_v$ (deg) & $+177 ^{+13} _{-16}$ & $+77 ^{+17} _{-20}$ & RV gradient direction (E. of N.) \\
\hline
  $\left<\feh\right>$ (dex, DR2.2) & $-1.77 ^{+0.08} _{-0.08}$ & $-2.10 ^{+0.08} _{-0.08}$ & Mean metallicity using full spectrum fit \tablenotemark{a} \\
  $\sigma_{\text{Fe}}$ (dex, DR2.2) & $+0.66 ^{+0.03} _{-0.03}$ & $+0.34 ^{+0.03} _{-0.03}$ & Metallicity dispersion \tablenotemark{a} \\
  $k_{\text{Fe}}$ (dex/deg, DR2.2) & $+0.10 ^{+0.09} _{-0.09}$ & $-0.05 ^{+0.20} _{-0.20}$ & Metallicity radial gradient \\
%   $\vhel$ ($\kms$) & $+288.9 ^{+0.4} _{-0.4}$ & $+89.3 ^{+0.3} _{-0.3}$ & Heliocentric radial velocity \\
%   %% T19: 290.9; C17/F19: 87.4/87.5
%   $\mu_{\alpha^*}$ ($\masyr$) & $-0.095 ^{+0.007} _{-0.007}$ & $-0.073 ^{+0.021} _{-0.021}$ & Heliocentric proper motion, RA $\cos \delta$ \\
%   $\mu_{\delta}$ ($\masyr$) & $+0.103 ^{+0.008} _{-0.008}$ & $-0.123 ^{+0.013} _{-0.013}$ & Heliocentric proper motion, Dec.\\
% \hline
%   $\vgsr$ (\kms) & $50.0^{+0.4}_{-0.4}$ & $-81.4 ^{+0.3} _{-0.3}$ & Galactic standard of rest, radial velocity \\
%   $\mu_{\alpha^*,\text{gsr}}$ (\masyr) & $-0.046^{+0.007}_{-0.007}$ & $+0.131 ^{+0.021} _{-0.021}$ & Galactic standard of rest, proper motion, RA $\cos \delta$\\
%   $\mu_{\delta,\text{gsr}}$ (\masyr) & $+0.178 ^{+0.008} _{-0.008}$ & $+0.118 ^{+0.013} _{-0.012}$ & Galactic standard of rest, proper motion, Dec\\
%   $\sigma_v$ (\kms) & $6.00^{+0.36}_{-0.35}$ & $+2.36 ^{+0.44} _{-0.30}$ & Radial velocity dispersion \\
%   %% T19: 5.7 +/- 1.1; C17/F19: 2.8 +/- 0.3, 2.7 +/- 0.5
%   $k_v$ (\kms/deg) & $3.73^{+0.65}_{-0.57}$ & $3.76 ^{+1.10} _{-1.08}$ & Linear radial velocity gradient\\
%   $k_v$ (\kms/kpc) & $1.62^{+0.28}_{-0.25}$ & $1.83 ^{+0.54}_{-0.52}$ & Linear radial velocity gradient\\
%   $\theta_v$ (deg) & $+177 ^{+13} _{-16}$ & $+77 ^{+17} _{-20}$ & RV gradient direction (E. of N.) \\
% \hline
%   $\left<\feh\right>$ (dex, DR2.2) & $-1.78 ^{+0.08} _{-0.08}$ & $-2.10 ^{+0.08} _{-0.08}$ & Mean metallicity using full spectrum fit \tablenotemark{a} \\
%   $\sigma_{\text{Fe}}$ (dex, DR2.2) & $+0.66 ^{+0.03} _{-0.03}$ & $+0.34 ^{+0.03} _{-0.03}$ & Metallicity dispersion \tablenotemark{a} \\
%   $k_{\text{Fe}}$ (dex/deg, DR2.2) & $+0.11 ^{+0.09} _{-0.09}$ & $-0.05 ^{+0.20} _{-0.20}$ & Metallicity radial gradient \\
\hline
  $\left<\feh\right>$ (dex, CaT) & $-1.92 \pm 0.03$ & $-2.26 \pm 0.03$ & Mean metallicity using calcium triplet EW \\
  $\sigma_{\text{Fe}}$ (dex, CaT) & $0.36 \pm 0.02$ & $0.25 \pm 0.03$ & Metallicity dispersion \\
\hline
  $N_{\text{mem}}$ & 284 & 141 & Number of clear member stars in our sample. \\
\hline
  $\sigma_v$, no $k_v$ (\kms) & $6.79^{+0.35}_{-0.33}$ & $2.75 ^{+0.51} _{-0.44}$ & Radial velocity dispersion without linear gradient \\
  $M_{\text{dyn}}$ ($M_\odot$) & TODO & TODO & Dynamical mass within half light radius \citep{Wolf10} \\
  $L_V$ ($L_\odot$) & & & Luminosity assuming $M_{V,\odot} = +4.83$ \\
  $M_\star$ ($M_\odot$) & & & Stellar mass assuming $M_\star/L_V = 2.2$ \\
  $M/L$ ($M_\odot/L_\odot$) & TODO & TODO & Mass to light ratio [xx do I use the luminosity within the half light radius?] \\
\enddata
\tablerefs{(1) \citealt{Torrealba19}, (2) \citealt{Torrealba16}, (3) \citealt{Vivas20}}
\tablenotetext{a}{The calcium triplet values are preferred over the full spectrum fit. The metallicity dispersion from the full spectrum fit is particularly influenced by a few outliers with inaccurate metallicities.}
\tablecomments{Values without references are measured in this work.}
\end{deluxetable*}

==> table.tex <==
\begin{table}[h]
    \centering
    \caption{Star 001 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 5.02 & --2.48 & 0.28 & 0.00 & 0.29 \\
Na I & 11.0 & 4.56 & --1.68 & 0.31 & 0.80 & 0.30 \\
Mg I & 12.0 & 5.2 & --2.4 & 0.18 & 0.08 & 0.24 \\
Al I & 13.0 & 4.25 & --2.2 & 0.49 & 0.28 & 0.47 \\
Si I & 14.0 & 5.67 & --1.84 & 0.33 & 0.65 & 0.34 \\
K I & 19.0 & 3.09 & --1.94 & 0.27 & 0.55 & 0.31 \\
Ca I & 20.0 & 4.13 & --2.21 & 0.16 & 0.28 & 0.23 \\
Sc II & 21.1 & 0.74 & --2.41 & 0.18 & 0.08 & 0.32 \\
Ti I & 22.0 & 2.65 & --2.3 & 0.23 & 0.18 & 0.26 \\
Ti II & 22.1 & 2.82 & --2.13 & 0.21 & 0.35 & 0.30 \\
V II & 23.1 & 1.65 & --2.28 & 0.43 & 0.21 & 0.52 \\
Cr I & 24.0 & 2.99 & --2.65 & 0.26 & --0.17 & 0.30 \\
Mn I & 25.0 & 2.38 & --3.05 & 0.22 & --0.57 & 0.29 \\
Fe II & 26.1 & 5.06 & --2.44 & 0.19 & 0.00 & 0.32 \\
Co I & 27.0 & 2.57 & --2.42 & 0.25 & 0.06 & 0.27 \\
Ni I & 28.0 & 3.89 & --2.33 & 0.25 & 0.15 & 0.28 \\
Sr II & 38.1 & 0.5 & --2.37 & 0.30 & 0.11 & 0.31 \\
Y II & 39.1 & --0.4 & --2.61 & 0.22 & --0.13 & 0.33 \\
Zr II & 40.1 & 0.31 & --2.27 & 0.26 & 0.21 & 0.38 \\
Ba II & 56.1 & --0.83 & --3.01 & 0.19 & --0.53 & 0.29 \\
La II & 57.1 & --1.0 & --2.1 & 0.24 & 0.38 & 0.36 \\
Eu II & 63.1 & --1.59 & --2.11 & 0.21 & 0.38 & 0.31 \\
C--H & 106.0 & 5.64 & --2.79 & 0.39 & --0.3 & 0.37 \\
C--N & 607.0 & 6.83 & --1.00 & 0.55 & 1.48 & 0.51 \\
Li I & 3.0 & 1.09 & $<$ 0.04 & -- & $<$ 2.53 & -- \\
O I & 8.0 & 7.84 & $<$ --0.85 & -- & $<$ 1.64 & -- \\
V I & 23.0 & 1.56 & $<$ --2.37 & -- & $<$ 0.11 & -- \\
Zn I & 30.0 & 2.86 & $<$ --1.70 & -- & $<$ 0.79 & -- \\
Dy II & 66.1 & --0.17 & $<$ --1.27 & -- & $<$ 1.21 & -- 
    \end{tabular}
    \label{tab:001}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 003 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.97 & --2.53 & 0.28 & 0.00 & 0.31 \\
Na I & 11.0 & 4.48 & --1.76 & 0.35 & 0.77 & 0.34 \\
Mg I & 12.0 & 5.27 & --2.33 & 0.18 & 0.20 & 0.26 \\
Al I & 13.0 & 4.21 & --2.24 & 0.56 & 0.29 & 0.55 \\
Si I & 14.0 & 5.44 & --2.07 & 0.37 & 0.47 & 0.38 \\
K I & 19.0 & 3.19 & --1.84 & 0.19 & 0.69 & 0.26 \\
Ca I & 20.0 & 4.21 & --2.13 & 0.19 & 0.40 & 0.27 \\
Sc II & 21.1 & 0.80 & --2.35 & 0.2 & 0.18 & 0.33 \\
Ti I & 22.0 & 2.62 & --2.33 & 0.26 & 0.2 & 0.29 \\
Ti II & 22.1 & 2.86 & --2.09 & 0.20 & 0.45 & 0.30 \\
Cr I & 24.0 & 2.94 & --2.7 & 0.28 & --0.17 & 0.31 \\
Cr II & 24.1 & 3.34 & --2.3 & 0.19 & 0.23 & 0.35 \\
Mn I & 25.0 & 2.71 & --2.72 & 0.31 & --0.19 & 0.35 \\
Fe II & 26.1 & 5.07 & --2.43 & 0.21 & 0.0 & 0.33 \\
Co I & 27.0 & 2.70 & --2.29 & 0.36 & 0.25 & 0.34 \\
Ni I & 28.0 & 3.76 & --2.46 & 0.22 & 0.07 & 0.28 \\
Sr II & 38.1 & 0.60 & --2.27 & 0.38 & 0.26 & 0.42 \\
Ba II & 56.1 & --0.60 & --2.78 & 0.19 & --0.25 & 0.30 \\
Eu II & 63.1 & --1.53 & --2.05 & 0.24 & 0.48 & 0.36 \\
C--H & 106.0 & 5.97 & --2.46 & 0.4 & 0.07 & 0.37 \\
C--N & 607.0 & 6.50 & --1.33 & 0.56 & 1.2 & 0.52 \\
O I & 8.0 & 7.2 & $<$ --1.49 & -- & $<$ 1.04 & -- \\
V I & 23.0 & 1.69 & $<$ --2.24 & -- & $<$ 0.29 & -- \\
V II & 23.1 & 2.34 & $<$ --1.59 & -- & $<$ 0.94 & -- \\
Zn I & 30.0 & 2.52 & $<$ --2.04 & -- & $<$ 0.49 & -- \\
Y II & 39.1 & --0.26 & $<$ --2.47 & -- & $<$ 0.06 & -- \\
Zr II & 40.1 & 0.9 & $<$ --1.68 & -- & $<$ 0.85 & -- \\
La II & 57.1 & --0.55 & $<$ --1.64 & -- & $<$ 0.89 & -- \\
    \end{tabular}
    \label{tab:003}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 005 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.77 & --2.73 & 0.27 & 0.0 & 0.24 \\
Na I & 11.0 & 4.28 & --1.96 & 0.36 & 0.77 & 0.29 \\
Mg I & 12.0 & 5.32 & --2.28 & 0.21 & 0.45 & 0.23 \\
Al I & 13.0 & 3.44 & --3.01 & 0.91 & --0.28 & 0.93 \\
Si I & 14.0 & 5.29 & --2.22 & 0.29 & 0.51 & 0.3 \\
K I & 19.0 & 2.91 & --2.12 & 0.21 & 0.61 & 0.23 \\
Ca I & 20.0 & 4.13 & --2.21 & 0.17 & 0.52 & 0.21 \\
Sc II & 21.1 & 0.36 & --2.79 & 0.18 & --0.06 & 0.26 \\
Ti I & 22.0 & 2.54 & --2.41 & 0.32 & 0.32 & 0.3 \\
Ti II & 22.1 & 2.54 & --2.41 & 0.24 & 0.32 & 0.29 \\
V II & 23.1 & 1.22 & --2.72 & 0.27 & 0.02 & 0.35 \\
Cr I & 24.0 & 2.76 & --2.87 & 0.33 & --0.14 & 0.32 \\
Cr II & 24.1 & 2.95 & --2.69 & 0.14 & 0.04 & 0.31 \\
Mn I & 25.0 & 2.26 & --3.17 & 0.3 & --0.44 & 0.31 \\
Fe II & 26.1 & 4.79 & --2.71 & 0.2 & 0.0 & 0.31 \\
Co I & 27.0 & 2.41 & --2.58 & 0.36 & 0.15 & 0.3 \\
Ni I & 28.0 & 3.73 & --2.49 & 0.28 & 0.24 & 0.29 \\
Sr II & 38.1 & 0.6 & --2.27 & 0.29 & 0.47 & 0.27 \\
Y II & 39.1 & --0.42 & --2.63 & 0.33 & 0.11 & 0.37 \\
Zr II & 40.1 & 0.19 & --2.39 & 0.27 & 0.34 & 0.36 \\
Ba II & 56.1 & --1.01 & --3.19 & 0.25 & --0.46 & 0.28 \\
La II & 57.1 & --1.42 & --2.52 & 0.31 & 0.21 & 0.33 \\
Eu II & 63.1 & --2.14 & --2.66 & 0.32 & 0.07 & 0.34 \\
Li I & 3.0 & 0.62 & $<$ --0.43 & -- & $<$ 2.31 & -- \\
O I & 8.0 & 7.13 & $<$ --1.56 & -- & $<$ 1.17 & -- \\
V I & 23.0 & 1.3 & $<$ --2.63 & -- & $<$ 0.1 & -- \\
Zn I & 30.0 & 2.48 & $<$ --2.08 & -- & $<$ 0.65 & -- \\
Dy II & 66.1 & --0.7 & $<$ --1.8 & -- & $<$ 0.93 & -- \\
C--H & 106.0 & 5.36 & $<$ --3.07 & -- & $<$ --0.34 & -- \\
C--N & 607.0 & 6.81 & $<$ --1.02 & -- & $<$ 1.72 & -- 
    \end{tabular}
    \label{tab:005}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 008 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.83 & --2.67 & 0.26 & 0.0 & 0.3 \\
Na I & 11.0 & 4.42 & --1.82 & 0.3 & 0.85 & 0.3 \\
Mg I & 12.0 & 5.23 & --2.37 & 0.2 & 0.3 & 0.27 \\
Al I & 13.0 & 3.89 & --2.56 & 0.77 & 0.11 & 0.78 \\
Si I & 14.0 & 5.45 & --2.06 & 0.3 & 0.61 & 0.32 \\
K I & 19.0 & 2.96 & --2.07 & 0.17 & 0.59 & 0.25 \\
Ca I & 20.0 & 4.1 & --2.24 & 0.15 & 0.42 & 0.25 \\
Sc II & 21.1 & 0.44 & --2.71 & 0.22 & --0.05 & 0.33 \\
Ti I & 22.0 & 2.64 & --2.31 & 0.24 & 0.36 & 0.28 \\
Ti II & 22.1 & 2.56 & --2.39 & 0.23 & 0.28 & 0.32 \\
V I & 23.0 & 1.25 & --2.68 & 0.31 & --0.02 & 0.35 \\
V II & 23.1 & 1.28 & --2.65 & 0.25 & 0.02 & 0.37 \\
Cr I & 24.0 & 2.76 & --2.88 & 0.21 & --0.21 & 0.27 \\
Cr II & 24.1 & 2.81 & --2.83 & 0.2 & --0.16 & 0.34 \\
Mn I & 25.0 & 2.33 & --3.1 & 0.26 & --0.43 & 0.32 \\
Fe II & 26.1 & 4.86 & --2.64 & 0.23 & 0.0 & 0.34 \\
Co I & 27.0 & 2.24 & --2.75 & 0.43 & --0.08 & 0.44 \\
Ni I & 28.0 & 3.49 & --2.73 & 0.23 & --0.06 & 0.28 \\
Zn I & 30.0 & 1.92 & --2.64 & 0.2 & 0.03 & 0.31 \\
Sr II & 38.1 & 0.18 & --2.69 & 0.32 & --0.02 & 0.37 \\
Y II & 39.1 & --0.88 & --3.09 & 0.24 & --0.42 & 0.34 \\
Zr II & 40.1 & 0.09 & --2.49 & 0.23 & 0.18 & 0.32 \\
Ba II & 56.1 & --0.78 & --2.96 & 0.22 & --0.29 & 0.3 \\
La II & 57.1 & --1.53 & --2.63 & 0.34 & 0.03 & 0.42 \\
Eu II & 63.1 & --2.25 & --2.77 & 0.23 & --0.1 & 0.31 \\
Dy II & 66.1 & --1.23 & --2.33 & 0.41 & 0.34 & 0.47 \\
C--H & 106.0 & 5.22 & --3.21 & 0.44 & --0.54 & 0.44 \\
Li I & 3.0 & 0.62 & $<$ --0.43 & -- & $<$ 2.24 & -- \\
O I & 8.0 & 7.09 & $<$ --1.6 & -- & $<$ 1.07 & -- \\
C--N & 607.0 & 6.4 & $<$ --1.43 & -- & $<$ 1.23 & -- 
    \end{tabular}
    \label{tab:008}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 016 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.85 & --2.65 & 0.21 & 0.0 & 0.23 \\
Na I & 11.0 & 4.4 & --1.84 & 0.29 & 0.81 & 0.26 \\
Mg I & 12.0 & 5.37 & --2.23 & 0.14 & 0.42 & 0.18 \\
Al I & 13.0 & 4.25 & --2.2 & 0.59 & 0.45 & 0.59 \\
Si I & 14.0 & 5.44 & --2.07 & 0.35 & 0.57 & 0.34 \\
K I & 19.0 & 3.08 & --1.95 & 0.17 & 0.7 & 0.2 \\
Ca I & 20.0 & 4.11 & --2.23 & 0.17 & 0.42 & 0.22 \\
Sc II & 21.1 & 0.65 & --2.5 & 0.11 & 0.15 & 0.23 \\
Ti I & 22.0 & 2.54 & --2.41 & 0.24 & 0.23 & 0.24 \\
Ti II & 22.1 & 2.64 & --2.31 & 0.15 & 0.34 & 0.23 \\
V I & 23.0 & 1.22 & --2.71 & 0.26 & --0.06 & 0.28 \\
V II & 23.1 & 1.42 & --2.51 & 0.19 & 0.13 & 0.28 \\
Cr I & 24.0 & 2.58 & --3.06 & 0.25 & --0.41 & 0.26 \\
Cr II & 24.1 & 2.9 & --2.74 & 0.17 & --0.1 & 0.29 \\
Mn I & 25.0 & 2.36 & --3.07 & 0.19 & --0.42 & 0.22 \\
Fe II & 26.1 & 4.85 & --2.65 & 0.18 & 0.0 & 0.28 \\
Co I & 27.0 & 2.47 & --2.52 & 0.26 & 0.13 & 0.25 \\
Ni I & 28.0 & 3.58 & --2.64 & 0.16 & 0.01 & 0.19 \\
Zn I & 30.0 & 2.19 & --2.36 & 0.17 & 0.28 & 0.26 \\
Sr II & 38.1 & 0.26 & --2.61 & 0.41 & 0.03 & 0.38 \\
Y II & 39.1 & --0.65 & --2.86 & 0.13 & --0.22 & 0.23 \\
Zr II & 40.1 & 0.02 & --2.56 & 0.21 & 0.08 & 0.31 \\
Ba II & 56.1 & --0.82 & --3.0 & 0.16 & --0.35 & 0.23 \\
La II & 57.1 & --1.87 & --2.97 & 0.33 & --0.33 & 0.37 \\
Eu II & 63.1 & --1.8 & --2.32 & 0.15 & 0.32 & 0.24 \\
Dy II & 66.1 & --0.95 & --2.05 & 0.26 & 0.59 & 0.32 \\
C--H & 106.0 & 5.65 & --2.78 & 0.34 & --0.13 & 0.32 \\
C--N & 607.0 & 6.39 & --1.44 & 0.52 & 1.2 & 0.48 \\
Li I & 3.0 & 0.76 & $<$ --0.29 & -- & $<$ 2.36 & -- \\
O I & 8.0 & 7.37 & $<$ --1.32 & -- & $<$ 1.33 & -- 
    \end{tabular}
    \label{tab:016}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 025 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.82 & --2.68 & 0.28 & 0.0 & 0.28 \\
Na I & 11.0 & 4.16 & --2.08 & 0.35 & 0.6 & 0.33 \\
Mg I & 12.0 & 5.4 & --2.2 & 0.19 & 0.48 & 0.23 \\
Al I & 13.0 & 2.96 & --3.49 & 0.49 & --0.82 & 0.55 \\
Si I & 14.0 & 5.4 & --2.11 & 0.32 & 0.57 & 0.31 \\
K I & 19.0 & 3.14 & --1.89 & 0.2 & 0.79 & 0.24 \\
Ca I & 20.0 & 4.1 & --2.24 & 0.17 & 0.44 & 0.23 \\
Sc II & 21.1 & 0.62 & --2.53 & 0.18 & 0.15 & 0.28 \\
Ti I & 22.0 & 2.57 & --2.38 & 0.25 & 0.29 & 0.25 \\
Ti II & 22.1 & 2.57 & --2.38 & 0.18 & 0.29 & 0.27 \\
V I & 23.0 & 1.41 & --2.52 & 0.4 & 0.15 & 0.39 \\
V II & 23.1 & 1.6 & --2.33 & 0.19 & 0.34 & 0.32 \\
Cr I & 24.0 & 2.95 & --2.69 & 0.32 & --0.01 & 0.33 \\
Mn I & 25.0 & 2.59 & --2.84 & 0.27 & --0.17 & 0.3 \\
Fe II & 26.1 & 4.8 & --2.7 & 0.17 & 0.0 & 0.31 \\
Co I & 27.0 & 2.42 & --2.57 & 0.39 & 0.1 & 0.38 \\
Ni I & 28.0 & 3.69 & --2.53 & 0.22 & 0.14 & 0.26 \\
Zn I & 30.0 & 2.21 & --2.35 & 0.24 & 0.33 & 0.31 \\
Sr II & 38.1 & --0.28 & --3.15 & 0.4 & --0.48 & 0.44 \\
Y II & 39.1 & --0.68 & --2.89 & 0.2 & --0.22 & 0.29 \\
Zr II & 40.1 & --0.1 & --2.68 & 0.3 & --0.0 & 0.36 \\
Ba II & 56.1 & --1.08 & --3.26 & 0.2 & --0.59 & 0.28 \\
La II & 57.1 & --1.69 & --2.79 & 0.38 & --0.12 & 0.45 \\
Eu II & 63.1 & --2.25 & --2.77 & 0.43 & --0.1 & 0.46 \\
Li I & 3.0 & 0.74 & $<$ --0.31 & -- & $<$ 2.37 & -- \\
O I & 8.0 & 7.39 & $<$ --1.3 & -- & $<$ 1.37 & -- \\
Dy II & 66.1 & --0.66 & $<$ --1.76 & -- & $<$ 0.91 & -- \\
C--H & 106.0 & 5.49 & $<$ --2.94 & -- & $<$ --0.26 & -- \\
C--N & 607.0 & 7.1 & $<$ --0.73 & -- & $<$ 1.95 & -- \\
    \end{tabular}
    \label{tab:025}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 026 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.91 & --2.59 & 0.24 & 0.0 & 0.24 \\
Na I & 11.0 & 4.76 & --1.48 & 0.31 & 1.11 & 0.28 \\
Mg I & 12.0 & 5.42 & --2.18 & 0.21 & 0.41 & 0.23 \\
Al I & 13.0 & 4.01 & --2.44 & 0.97 & 0.15 & 0.95 \\
Si I & 14.0 & 5.24 & --2.27 & 0.3 & 0.32 & 0.29 \\
K I & 19.0 & 2.94 & --2.09 & 0.26 & 0.51 & 0.29 \\
Ca I & 20.0 & 4.22 & --2.12 & 0.2 & 0.47 & 0.24 \\
Sc II & 21.1 & 0.62 & --2.53 & 0.21 & 0.07 & 0.32 \\
Ti I & 22.0 & 2.62 & --2.33 & 0.29 & 0.27 & 0.28 \\
Ti II & 22.1 & 2.64 & --2.31 & 0.17 & 0.29 & 0.27 \\
V II & 23.1 & 1.56 & --2.37 & 0.26 & 0.22 & 0.36 \\
Cr I & 24.0 & 2.52 & --3.12 & 0.28 & --0.53 & 0.29 \\
Cr II & 24.1 & 3.17 & --2.47 & 0.17 & 0.13 & 0.31 \\
Mn I & 25.0 & 2.35 & --3.08 & 0.24 & --0.49 & 0.28 \\
Fe II & 26.1 & 4.98 & --2.52 & 0.21 & 0.0 & 0.31 \\
Co I & 27.0 & 2.36 & --2.63 & 0.4 & --0.03 & 0.38 \\
Ni I & 28.0 & 3.56 & --2.66 & 0.22 & --0.07 & 0.24 \\
Zn I & 30.0 & 1.95 & --2.61 & 0.28 & --0.02 & 0.36 \\
Sr I & 38.0 & 0.99 & --1.88 & 0.28 & 0.71 & 0.3 \\
Sr II & 38.1 & 1.06 & --1.81 & 0.24 & 0.79 & 0.26 \\
Y II & 39.1 & --0.04 & --2.25 & 0.23 & 0.34 & 0.31 \\
Zr II & 40.1 & 0.53 & --2.05 & 0.44 & 0.54 & 0.55 \\
Ba II & 56.1 & 0.94 & --1.24 & 0.24 & 1.35 & 0.25 \\
La II & 57.1 & --0.45 & --1.55 & 0.17 & 1.04 & 0.28 \\
Eu II & 63.1 & --1.8 & --2.32 & 0.2 & 0.27 & 0.27 \\
C--H & 106.0 & 5.98 & --2.45 & 0.33 & 0.14 & 0.31 \\
C--N & 607.0 & 7.37 & --0.46 & 0.52 & 2.13 & 0.47 \\
Li I & 3.0 & 0.58 & $<$ --0.47 & -- & $<$ 2.12 & -- \\
O I & 8.0 & 7.22 & $<$ --1.47 & -- & $<$ 1.13 & -- \\
V I & 23.0 & 1.29 & $<$ --2.64 & -- & $<$ --0.04 & -- \\
Dy II & 66.1 & 0.19 & $<$ --0.91 & -- & $<$ 1.69 & -- 
    \end{tabular}
    \label{tab:026}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 033 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 4.94 & --2.56 & 0.28 & 0.0 & 0.31 \\
Na I & 11.0 & 4.6 & --1.64 & 0.34 & 0.92 & 0.33 \\
Mg I & 12.0 & 5.43 & --2.17 & 0.21 & 0.39 & 0.26 \\
Al I & 13.0 & 4.38 & --2.07 & 0.99 & 0.49 & 0.96 \\
Si I & 14.0 & 5.43 & --2.08 & 0.28 & 0.48 & 0.31 \\
K I & 19.0 & 3.09 & --1.94 & 0.25 & 0.62 & 0.29 \\
Ca I & 20.0 & 4.16 & --2.18 & 0.22 & 0.38 & 0.29 \\
Sc II & 21.1 & 0.56 & --2.59 & 0.22 & --0.03 & 0.35 \\
Ti I & 22.0 & 2.46 & --2.49 & 0.24 & 0.07 & 0.27 \\
Ti II & 22.1 & 2.61 & --2.34 & 0.23 & 0.22 & 0.34 \\
V I & 23.0 & 1.21 & --2.72 & 0.21 & --0.16 & 0.3 \\
V II & 23.1 & 1.53 & --2.4 & 0.25 & 0.16 & 0.4 \\
Cr I & 24.0 & 2.91 & --2.73 & 0.29 & --0.17 & 0.32 \\
Cr II & 24.1 & 3.01 & --2.63 & 0.19 & --0.07 & 0.35 \\
Mn I & 25.0 & 2.29 & --3.14 & 0.18 & --0.58 & 0.28 \\
Fe II & 26.1 & 4.94 & --2.56 & 0.17 & 0.0 & 0.31 \\
Co I & 27.0 & 2.52 & --2.47 & 0.33 & 0.09 & 0.37 \\
Ni I & 28.0 & 3.76 & --2.46 & 0.24 & 0.1 & 0.27 \\
Zn I & 30.0 & 2.22 & --2.34 & 0.22 & 0.22 & 0.33 \\
Sr II & 38.1 & 0.29 & --2.58 & 0.34 & --0.02 & 0.39 \\
Y II & 39.1 & --0.62 & --2.83 & 0.2 & --0.27 & 0.33 \\
Zr II & 40.1 & 0.05 & --2.53 & 0.27 & 0.03 & 0.41 \\
Ba II & 56.1 & --0.79 & --2.97 & 0.2 & --0.41 & 0.31 \\
Eu II & 63.1 & --2.08 & --2.6 & 0.26 & --0.04 & 0.38 \\
Dy II & 66.1 & --0.35 & --1.45 & 0.44 & 1.11 & 0.47 \\
C--H & 106.0 & 5.47 & --2.96 & 0.35 & --0.4 & 0.37 \\
C--N & 607.0 & 6.24 & --1.59 & 0.74 & 0.97 & 0.7 \\
Li I & 3.0 & 0.3 & $<$ --0.75 & -- & $<$ 1.81 & -- \\
O I & 8.0 & 6.47 & $<$ --2.22 & -- & $<$ 0.34 & -- \\
La II & 57.1 & --1.49 & $<$ --2.59 & -- & $<$ --0.03 & -- 
    \end{tabular}
    \label{tab:033}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 184 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 5.1 & --2.4 & 0.21 & 0.0 & 0.2 \\
Na I & 11.0 & 4.16 & --2.08 & 0.36 & 0.32 & 0.29 \\
Mg I & 12.0 & 5.72 & --1.88 & 0.26 & 0.51 & 0.24 \\
Al I & 13.0 & 3.19 & --3.26 & 1.08 & --0.86 & 1.04 \\
Si I & 14.0 & 5.43 & --2.08 & 0.32 & 0.32 & 0.31 \\
K I & 19.0 & 3.47 & --1.56 & 0.3 & 0.84 & 0.26 \\
Ca I & 20.0 & 4.33 & --2.01 & 0.19 & 0.39 & 0.2 \\
Sc II & 21.1 & 0.94 & --2.21 & 0.24 & 0.19 & 0.33 \\
Ti I & 22.0 & 2.85 & --2.1 & 0.27 & 0.29 & 0.22 \\
Ti II & 22.1 & 3.13 & --1.82 & 0.2 & 0.58 & 0.27 \\
V I & 23.0 & 1.5 & --2.43 & 0.31 & --0.03 & 0.3 \\
V II & 23.1 & 1.8 & --2.13 & 0.26 & 0.27 & 0.32 \\
Cr I & 24.0 & 3.12 & --2.52 & 0.24 & --0.12 & 0.19 \\
Cr II & 24.1 & 3.39 & --2.25 & 0.16 & 0.15 & 0.29 \\
Mn I & 25.0 & 2.52 & --2.91 & 0.19 & --0.51 & 0.2 \\
Fe II & 26.1 & 5.11 & --2.39 & 0.14 & 0.0 & 0.26 \\
Co I & 27.0 & 2.9 & --2.09 & 0.31 & 0.31 & 0.29 \\
Ni I & 28.0 & 3.8 & --2.42 & 0.27 & --0.02 & 0.26 \\
Zn I & 30.0 & 2.28 & --2.28 & 0.13 & 0.12 & 0.24 \\
Sr II & 38.1 & 0.83 & --2.04 & 0.19 & 0.36 & 0.23 \\
Y II & 39.1 & --0.3 & --2.51 & 0.19 & --0.11 & 0.28 \\
Zr II & 40.1 & 0.59 & --1.99 & 0.31 & 0.41 & 0.42 \\
Ba II & 56.1 & --0.51 & --2.69 & 0.17 & --0.29 & 0.25 \\
La II & 57.1 & --1.6 & --2.7 & 0.21 & --0.3 & 0.29 \\
Eu II & 63.1 & --1.75 & --2.27 & 0.17 & 0.13 & 0.25 \\
Dy II & 66.1 & --0.94 & --2.04 & 0.36 & 0.36 & 0.4 \\
C--H & 106.0 & 5.49 & --2.94 & 0.38 & --0.54 & 0.36 \\
C--N & 607.0 & 6.06 & --1.77 & 0.44 & 0.63 & 0.41 \\
Li I & 3.0 & 0.04 & $<$ --1.01 & -- & $<$ 1.39 & -- \\
O I & 8.0 & 7.45 & $<$ --1.24 & -- & $<$ 1.16 & -- 
    \end{tabular}
    \label{tab:184}
\end{table}

\begin{table}[h]
    \centering
    \caption{Star 576 Abundances}
    \begin{tabular}{ccccccc}
Element & Species & $\log \epsilon$ & [X/H] & $e_{\text{[X/H]}}$ & [X/Fe] & $e_{\text{[X/Fe]}}$ \\
\hline & & & & & & \\
Fe I & 26.0 & 5.02 & --2.48 & 0.21 & 0.0 & 0.23 \\
Na I & 11.0 & 4.49 & --1.75 & 0.3 & 0.73 & 0.27 \\
Mg I & 12.0 & 5.36 & --2.24 & 0.17 & 0.24 & 0.2 \\
Al I & 13.0 & 4.34 & --2.11 & 0.76 & 0.37 & 0.74 \\%& 13.0 & 4.44 & --2.01 & 0.47 & 1.04 & 0.74 \\
Si I & 14.0 & 5.63 & --1.88 & 0.27 & 0.6 & 0.27 \\
K I & 19.0 & 3.28 & --1.75 & 0.19 & 0.74 & 0.21 \\
Ca I & 20.0 & 4.17 & --2.17 & 0.14 & 0.31 & 0.19 \\
Sc II & 21.1 & 0.74 & --2.41 & 0.12 & 0.08 & 0.25 \\
Ti I & 22.0 & 2.61 & --2.34 & 0.2 & 0.14 & 0.2 \\
Ti II & 22.1 & 2.84 & --2.11 & 0.17 & 0.37 & 0.25 \\
V I & 23.0 & 1.37 & --2.56 & 0.23 & --0.08 & 0.25 \\
V II & 23.1 & 1.66 & --2.27 & 0.21 & 0.21 & 0.32 \\
Cr I & 24.0 & 2.96 & --2.68 & 0.2 & --0.2 & 0.21 \\
Cr II & 24.1 & 3.22 & --2.42 & 0.12 & 0.06 & 0.26 \\
Mn I & 25.0 & 2.55 & --2.88 & 0.15 & --0.4 & 0.2 \\
Fe II & 26.1 & 5.05 & --2.45 & 0.15 & 0.0 & 0.27 \\
Co I & 27.0 & 2.74 & --2.25 & 0.21 & 0.23 & 0.23 \\
Ni I & 28.0 & 3.81 & --2.41 & 0.23 & 0.07 & 0.26 \\
Zn I & 30.0 & 2.25 & --2.31 & 0.14 & 0.17 & 0.24 \\
Sr II & 38.1 & 0.42 & --2.45 & 0.29 & 0.04 & 0.3 \\
Y II & 39.1 & --0.49 & --2.7 & 0.13 & --0.22 & 0.25 \\
Zr II & 40.1 & 0.38 & --2.2 & 0.19 & 0.29 & 0.3 \\
Ba II & 56.1 & --0.68 & --2.86 & 0.16 & --0.38 & 0.25 \\
La II & 57.1 & --1.42 & --2.52 & 0.16 & --0.04 & 0.26 \\
Eu II & 63.1 & --1.59 & --2.11 & 0.14 & 0.37 & 0.24 \\
Dy II & 66.1 & --0.97 & --2.07 & 0.27 & 0.41 & 0.35 \\
C--H & 106.0 & 5.3 & --3.13 & 0.3 & --0.65 & 0.3 \\
C--N & 607.0 & 6.66 & --1.17 & 0.49 & 1.31 & 0.46 \\
O I & 8.0 & 7.35 & $<$ --1.34 & -- & $<$ 1.14 & -- 
    \end{tabular}
    \label{tab:576}
\end{table}
